Reducing Meshing Requirements for Electrostatic Problems using a Galerkin Boundary Element Method

This work focuses on model preparation for electrostatic simulations of CAD designs to realize a rapid virtual prototyping concept. We present a boundary element method (BEM) allowing discontinuous fields between surfaces. The corresponding edges of the CAD model are enhanced with the data required to integrate over non-conforming elements. Finally, we generate a mesh for each CAD surface. The approach is verified via numerical experiments and shows excellent agreement with conforming BEM results.

==> mycommands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Algorithms
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\RequirePackage{algorithmic} %% \usepackage[noend]{algorithmic}

%% Algorithm comment style
\newcommand{\store}{=} 	% symbol for storing with in algorithm
\newcommand{\myinsert}{\leftarrow} 	% symbol for insertions with in algorithm
% \renewcommand{\algorithmiccomment}[1]{\hspace{1cm} // #1} 
\renewcommand{\algorithmiccomment}[1]{\hspace{1cm}$\vartriangleright$ #1}

%% Algorithm environment
\newenvironment{myalgorithm}%[2]%
{
  % #1=caption #2=label
%   \begin{algorithm}
%     \caption{#1}
%     \label{#2}
    \begin{algorithmic}[1]
}   
{
\end{algorithmic}
% \end{algorithm}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Include Tikz pictures
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\RequirePackage{tikz} %% also include \usetikzlibrary{external}
%% option:
% If \tikzOff is defined in main.tex figure "filename.pdf" is 
% included directly with no externalize.
%% provide default paths (if not already defined elsewhere)
\providecommand{\MainPath}{.}
\providecommand{\TikzPath}{\MainPath/tikz}
\providecommand{\DataPath}{\MainPath/data}
\providecommand{\PicsPath}{\MainPath/pics}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% input of figures computed by Tikz
%
% filename=#1, (without .tex extension)
% size=#2, 
% caption=#3, 
% label=#4, 
%
%% Example call:
% \begin{figure}
%     \tikzfig{TikzFileName}{1.0}{Dummy caption}{fig:example}
% \end{figure}
%
\ifdefined\tikzOff
\newcommand{\tikzfig}[4]{
    \centering
    \includegraphics{#1} % note: set \graphicspath{} to file location
    \caption{#3}
    \label{#4}
}
\else
\newcommand{\tikzfig}[4]{
  \centering
  \def\tkzscale{#2}
  \tikzsetnextfilename{#1}
  \input{\TikzPath/#1}
  \caption{#3}
  \label{#4}
}
\fi

%% add Tikz Subfigures 
%
% path/filename=#1, 
% size=#2, 
% subcaption=#3, 
% label=#4
%
%% Example call
% \begin{figure}[t]
%     \centering
%     \begin{minipage}[b]{0.48\textwidth}
%         \tikzsubfig{tikzA.tex}{1.0}{Subcaption A}{fig:A}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.48\textwidth}
%         \tikzsubfig{tikzB.tex}{1.0}{Subcaption B}{fig:B}
%     \end{minipage}
%     \caption{Caption}
%     \label{fig:A-B}
% \end{figure}
%
\ifdefined\tikzOff
\newcommand{\tikzsubfig}[4]{
    \centering
    \includegraphics{#1} % note: set \graphicspath{} to file location
    \subcaption{#3}
    \label{#4}
}
\else
\newcommand{\tikzsubfig}[4]{
    \def\tkzscale{#2}
    \centering
    \tikzsetnextfilename{#1}
    \input{\TikzPath/#1}
    \subcaption{#3}
    \label{#4}
}
\fi

% % dirtikzfolder=#1 datafolder=#2 file=#3, size=#4, overlaynumber (starting with 0)=#5
% % \tikzfignocaption{tikz/}{data}{filename}{1.0}[0]
% \newcommandx{\tikzfignocaption}[5][5=0]{
%   \begin{figure}[ht]%[htb!]
%     \def\tkzscale{#4}
%     \def\dirtikz{\MainPath/#1} % define tikz directory
%     \def\dirdata{\MainPath/#2} % define data directory
%     \centering
%     \tikzsetnextfilename{#3-figure#5}  
%     \input{\dirtikz #3}
%   \end{figure}
% }

\makeatletter
%%% NOTE: the maximal number of slides must be given at the end of each \tikzfigforbeamer command
%%% overlay of the tikz fig with higher number will be ignored!!
\newcommand*{\overlaynumber}{\number\beamer@slideinframe}
\makeatother
\RequirePackage{xargs}
\RequirePackage{ifthen}
%% TikZ Figure with absolute scaling
\newcommandx{\tikzfigforbeamer}[6][1=tikz/,2=data]{
  % dirtikzfolder=#1, datafolder=#2, file=#3, size=#4, maximal total number of slides=#5, #6==0 use pdf directly; compute tikz otherwise
  \ifdefined\tikzTmpPDFOff
    \onslide<-#5>{ 
      \pgfmathsetmacro{\FigNumber}{int(\overlaynumber-1)}     
      % \tikzfignocaption{#1}{#2}{#3}{#4}[\FigNumber]
      \begin{figure}[ht]%[htb!]
          \def\tkzscale{#4}
          \def\dirtikz{\MainPath/#1} % define tikz directory
          \def\dirdata{\MainPath/#2} % define data directory
          \centering
          \pgfmathsetmacro{\FigNumber}{int(\overlaynumber-1)}
          \tikzsetnextfilename{#3-figure\FigNumber}  
          \input{\dirtikz #3}
      \end{figure}
    }
  \else
    \ifthenelse{\equal{#6}{0}}{
        \onslide<-#5>{
          \pgfmathsetmacro{\FigNumber}{int(\overlaynumber-1)}
          \begin{figure}[ht]
              \centering
              % \pgfmathsetmacro{\FigNumber}{int(\overlaynumber-1)}
              \includegraphics[scale=1.0]{#3-figure\FigNumber}
          \end{figure}
        }
    }{%
        \onslide<-#5>{     
          \pgfmathsetmacro{\FigNumber}{int(\overlaynumber-1)}     
            % \tikzfignocaption{#1}{#2}{#3}{#4}[\FigNumber]
            \begin{figure}[ht]%[htb!]
              \def\tkzscale{#4}
              \def\dirtikz{\MainPath/#1} % define tikz directory
              \def\dirdata{\MainPath/#2} % define data directory
              \centering
              \pgfmathsetmacro{\FigNumber}{int(\overlaynumber-1)}
              \tikzsetnextfilename{#3-figure\FigNumber}  
              \input{\dirtikz #3}
            \end{figure}
        } 
    }
  \fi
}


%% TikZ Figure with absolute scaling
\newcommandx{\tikzfigforbeamerstatic}[5][1=tikz/,2=data]{
  % dirtikzfolder=#1, datafolder=#2, file=#3, size=#4, #5==0 use pdf directly; compute tikz otherwise
  \ifdefined\tikzTmpPDFOff 
    % \tikzfignocaption{#1}{#2}{#3}{#4}
    \begin{figure}[ht]%[htb!]
      \def\tkzscale{#4}
      \def\dirtikz{\MainPath/#1} % define tikz directory
      \def\dirdata{\MainPath/#2} % define data directory
      \centering
      \tikzsetnextfilename{#3-figure0}  
      \input{\dirtikz #3}
    \end{figure}
  \else
    \ifthenelse{\equal{#5}{0}}{
      \begin{figure}[ht]
          \centering
          \includegraphics[scale=1.0]{#3-figure0}
      \end{figure}
    }{% 
      \begin{figure}[ht]%[htb!]
        \def\tkzscale{#4}
        \def\dirtikz{\MainPath/#1} % define tikz directory
        \def\dirdata{\MainPath/#2} % define data directory
        \centering
        \tikzsetnextfilename{#3-figure0}  
        \input{\dirtikz #3}
      \end{figure}   
      % \tikzfignocaption{#1}{#2}{#3}{#4}
        % \begin{figure}[ht]%[htb!]
        %     \def\tkzscale{#2}
        %     \def\dirtikz{\MainPath/tikz/} % define tikz directory
        %     \def\dirdata{\MainPath/data} % define data directory
        %     \centering
        %     \tikzsetnextfilename{#1-figure0}  
        %     \input{\dirtikz #1}
        % \end{figure}
    } 
  \fi
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Define table style
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newenvironment{mytableBeamer}[4]%
{
  % #1=caption #2=label #3=table layout #4=position
  \begin{table}[#4]%[htb!]
    % \caption{#1}
    % \label{tab:#2}
%     \def\mycap{#1}
%     \def\mylabel{tab:#2}
    \centering
    \begin{tabular}{#3}
      \toprule
%       #4 \\ 
%       \midrule
%       \hline%\noalign{\smallskip}
}
{
  %\noalign{\smallskip}
%   \hline
  \bottomrule
  \end{tabular}
%   \caption{\mycap}
%   \label{\mylabel}
  \end{table}
}
\newcommand{\mytableheader}[1]{
  % #1=header without line breaks (i.e. ' 1.col & 2.col & 3.col ' )
       #1 \\ \midrule
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% reduce left margin for a slide
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\Wider[2][3em]{%
\makebox[\linewidth][c]{%
  \begin{minipage}{\dimexpr\textwidth+#1\relax}
  \raggedright#2
  \end{minipage}%
  }%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% colors used in the template 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\colorlet{TUGgray}{black!15}
\definecolor{TUGred}{RGB}{247,1,70}
\definecolor{IFBblue}{RGB}{51,112,169}
\definecolor{Mech_blau}{RGB}{0,103,173}

\definecolor{mygreen}{rgb}{0,.5,0}
\newcommand{\inred}    {\color{TUGred}}
\newcommand{\ingreen}  {\color{mygreen}}
\newcommand{\inblue}   {\color{Mech_blau}}
\newcommand{\ingray}   {\color{gray}}
% \newcommand{\inlightblue}  {\color{blue!60}}
\newcommand{\inolive}  {\color{olive}}
% \newcommand{\inpurple} {\color{purple}}
\newcommand{\inpurple} {\color{IFBblue}}
\newcommand{\inlightgray}   {\color{gray!30}}
\newcommand{\intug} {\color{TUGred}}
\newcommand{\inrot}[1]{\color{TUGred}#1\color{black}}
\newcommand{\inblau}[1]{\color{Mech_blau}#1\color{black}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% listings styles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mySetlstColor}{darkgray!60} 
\newcommand{\mySetlstStyleSTEP}{
    \lstset{language=C++,
        keepspaces=true,
%         moredelim=[is][\color{black}\underbar]{|}{|}, TUGred
        moredelim=[is][\color{black}]{|}{|},
%         moredelim=[is][\color{basisColor1}]{|-}{-|},
%         moredelim=[is][\color{basisColor1}\bf]{||}{||},
        print=true,
        fontadjust=true,
        columns=fixed,
%         morekeywords={48,},
%         keywordstyle=\bf\color{red},
%         commentstyle=\bf\ttfamily\scriptsize\color{\mySetlstColor},
%         basicstyle=\ttfamily\scriptsize\color{\mySetlstColor},
        commentstyle=\bf\ttfamily\tiny\color{\mySetlstColor},
        basicstyle=\ttfamily\tiny\color{\mySetlstColor},
        basewidth=0.52em
    }    
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% highlight text, e.g., in equations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newcommand{\myhighlight}[1]{%
%   \colorbox{red!50}{$\displaystyle#1$}}
\newcommand{\myhighlight}[1]{%
    \tikzset{external/export=false}
    \tikz[baseline]{
        \node[fill=red!50, rounded corners=1mm,anchor=base] (t2)
        {$#1$};
    }
}
% \newcommand{\highlight}[1]{\colorbox{red!50}{$\displaystyle#1$}}
	



\newcommand{\myhref}[2]{\href{#1}{\textcolor{Mech_blau}{#2}}}


==> mytikzcommands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % mytikzcomments.tex
% %
% % 	requires:		\usepackage{tikz}
% % 				\usepackage{forloop}
% % 				\usepackage{arrayjobx}
% %
\RequirePackage{tikz}
\RequirePackage{pgfplots}  
\RequirePackage{forloop} 
\RequirePackage{arrayjobx} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% compatibility
\pgfplotsset{compat=1.10}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% externalize tikz-figures as graphics
\usetikzlibrary{external}
\tikzexternalize[optimize command away={\includepdf,\includegraphics}] %externalize ignores \includepdf objects
% \tikzset{external/optimize command away=\includegraphics}
% \tikzexternalize[mode=list and make,prefix=tmp/]
% \tikzset{external/mode=list and make}
\tikzsetexternalprefix{tmp/}
% \tikzexternaldisable

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% TikZ additional packages
\usetikzlibrary{positioning,calc,intersections,arrows,3d,fit}
% \usetikzlibrary{shapes,snakes,spy}
\usetikzlibrary{shapes,spy,fit}
% \usepgfplotslibrary{patchplots}
% \usetikzlibrary{matrix,chains,scopes,fit,decorations.pathmorphing} % for sim chain
% \usetikzlibrary{shapes.geometric,shapes.arrows,decorations.pathmorphing}
% \usetikzlibrary{matrix,chains,scopes,positioning,arrows,fit}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% PGF Plots additional packages
\usepgfplotslibrary{groupplots}
% \usepgfplotslibrary{fillbetween}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Advanced clipping option 
%%% source: https://tex.stackexchange.com/questions/12010/how-can-i-invert-a-clip-selection-within-tikz
%%% usage: 
%%% \begin{pgfinterruptboundingbox}
%%% \path [clip] (A) -- (B) -- (C) -- cycle [reverseclip];
%%% \end{pgfinterruptboundingbox}
 
\tikzstyle{reverseclip}=[insert path={(current page.north east) --
    (current page.south east) --
    (current page.south west) --
    (current page.north west) --
    (current page.north east)}
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Font size in plots and graphics
\def\pgfplotfontsize{\scriptsize}
\def\pgfplotfontsizetitle{\scriptsize}
\def\pgfplotfontsizetiny{\scriptsize}
\def\pgfplotfontsizelegend{\small}
\def\tikzfontsize{\small}
\def\tikzfontsizesmall{\scriptsize}
\def\tikzfontsizetiny{\tiny}

\pgfplotsset{
  mystyle/.style ={%
    grid = major,
%     grid = none,
    every tick label/.append style={font=\pgfplotfontsize},
    every axis label/.append style={font=\pgfplotfontsize},
    legend style={font=\pgfplotfontsize},
    label style={font=\pgfplotfontsize},
    title style={font=\pgfplotfontsizetitle},
%       \pgfkeys{%
    /pgf/number format/set thousands separator = {}, % 1,000 -> 1000
%   }
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Custom drawing colors
% \definecolor{drawblue} {RGB}{87,117,225}
\colorlet{drawblue}      {blue!80!white}
% \definecolor{drawred}{RGB}{229,112,88}
\colorlet{drawred}       {red!80!white}
\colorlet{drawgray}      {gray}
% \definecolor{drawgreen}  {RGB}{0,.5,0}
\definecolor{drawgreen}  {RGB}{44,162,95}
% \definecolor{drawgreen}  {RGB}{49,163,84}
% \colorlet{drawgreen}  {olive}
\colorlet{drawpurple}    {purple}
\colorlet{draworange}    {orange}
\colorlet{drawlime}      {lime!80!black}
\colorlet{drawartichoke} {yellow!60!black}
\colorlet{TUGgray}{black}
\definecolor{TUGred}{RGB}{247,1,70}
\definecolor{IFBblue}{RGB}{51,112,169}
% \definecolor{UTorange}{RGB}{191,87,0}
% \definecolor{UTblue}{RGB}{0,95,134}
\colorlet{UTorange}{red!75!black} % only for trimmingTimeline...
\colorlet{UTblue}{rgb:red,1;green,2;blue,5} % only for trimmingTimeline...
\definecolor{UTgreen}{RGB}{67,105,91}
\definecolor{UTgray}{RGB}{51,63,72}
\definecolor{UTyellow}{RGB}{242,169,0}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Custom basisfunction colors
\definecolor{basisColor1}{RGB}{59,76,192}
\definecolor{basisColor2}{RGB}{87,117,225}
\definecolor{basisColor3}{RGB}{119,154,247}
\definecolor{basisColor4}{RGB}{152,185,255}
\definecolor{basisColor5}{RGB}{184,208,249}
% \definecolor{basisColor6}{RGB}{213,219,230} % original settings
% \definecolor{basisColor7}{RGB}{236,211,197} % original settings
\definecolor{basisColor6}{RGB}{195,209,230}	% changed for printing
\definecolor{basisColor7}{RGB}{247,200,190}	% changed for printing
\definecolor{basisColor8}{RGB}{247,187,160}
\definecolor{basisColor9}{RGB}{244,154,123}
\definecolor{basisColor10}{RGB}{229,112,88}
\definecolor{basisColor11}{RGB}{203,62,56}
\definecolor{basisColor12}{RGB}{180,4,38}

\definecolor{basisColor8sw}{RGB} {189,189,189}
\definecolor{basisColor9sw}{RGB} {150,150,150}
\definecolor{basisColor10sw}{RGB}{115,115,115}
% \definecolor{basisColor11sw}{RGB}{82,82,82}
\definecolor{basisColor11sw}{RGB}{91,91,91}
\definecolor{basisColor12sw}{RGB}{37,37,37}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Custom plot colors and style

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Initial set 0 (standard TikZ)
\colorlet{myblue}    {blue}
\colorlet{myred}     {red}
% \definecolor{mygreen} {RGB}{44,162,95}
\colorlet{mygreen}   {drawgreen}
\colorlet{mypurple}  {purple}
\colorlet{myorange}  {orange}


%%% Set 1 - dark colors
%%% http://colorbrewer2.org, number of data classes=3, middle color
%% \definecolor{myblue}  {RGB}{43,140,190}
% \definecolor{myblue}  {RGB}{43,140,190}
% \definecolor{myred}   {RGB}{227,74,51}
% \definecolor{mygreen} {RGB}{44,162,95}
% \definecolor{mypurple}{RGB}{197,27,138}
% \definecolor{myorange}{RGB}{217,95,14}

%%% Set 2 - light colors
%%% http://colorbrewer2.org, number of data classes=3, middle color
% \definecolor{myblue}  {RGB}{166,189,219}
% \definecolor{myred}   {RGB}{253,187,132}
% \definecolor{mygreen} {RGB}{153,216,201}
% \definecolor{mypurple} {RGB}{250,159,181}
% \definecolor{myorange}{RGB}{254,196,79 }


%%% Cycle lists for plots


%%% Cyclelist 1 (custom)
% \pgfplotscreateplotcyclelist{mycyclelist}{
%   myblue,    every mark/.append style={solid, fill=.},mark=*          \\%
%   myred,     every mark/.append style={solid, fill=.},mark=square*     \\%
%   mygreen,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
%   mypurple,  every mark/.append style={solid, fill=.},mark=diamond*    \\%
%   % myorange,  every mark/.append style={solid, fill=.},mark=star    \\%
% }

% \pgfplotscreateplotcyclelist{mycyclelistcompare}{
%   myblue,    dashed            \\%
%   myred,     dotted            \\%
%   mygreen,   dashdotted        \\%
%   mypurple,  dashdotdotted     \\%
%   myblue,    only marks,   every mark/.append style={solid, fill=.},mark=*          \\%
%   myred,     only marks,   every mark/.append style={solid, fill=.},mark=square*     \\%
%   mygreen,   only marks,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
%   mypurple,  only marks,   every mark/.append style={solid, fill=.},mark=diamond*    \\%
% }

%%% Cyclelist 2 (TikZ exotic)
% \pgfplotscreateplotcyclelist{mycyclelist}{
%   teal,    every mark/.append style={solid, fill=.},mark=*           \\%
%   orange,  every mark/.append style={solid, fill=.},mark=square*     \\%
%   cyan,    every mark/.append style={solid, fill=.},mark=triangle*   \\%
%   red,     every mark/.append style={solid, fill=.},mark=diamond*    \\%
%   % lime,  every mark/.append style={solid, fill=.},mark=diamond*    \\%
% }

% %%% Cyclelist 3 (TikZ standard)
% \pgfplotscreateplotcyclelist{mycyclelist}{
% %     \pgfplotscreateplotcyclelist{color}{%
% blue,every mark/.append style={fill=blue!80!black},mark=*\\%
% red,every mark/.append style={fill=red!80!black},mark=square*\\%
% brown!60!black,every mark/.append style={fill=brown!80!black},mark=otimes*\\%
% black,mark=star\\%
% blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
% red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
% brown!60!black,densely dashed,every mark/.append style={
% solid,fill=brown!80!black},mark=square*\\%
% black,densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
% blue,densely dashed,mark=star,every mark/.append style=solid\\%
% red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*\\%
% % }
% %   blue,    every mark/.append style={solid, fill=.},mark=*           \\%
% %   red,     every mark/.append style={solid, fill=.},mark=square*     \\%
% %   brown,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
% %   black,   every mark/.append style={solid, fill=.},mark=diamond*    \\%
% }

%%% Cyclelist 4 (red styles)

% % \ifthenelse{\boolean{isbook}}{ 
% % % \definecolor{basisColor11new}{RGB}{203,80,56}
% % 
% % %% gray styles
% % \pgfplotscreateplotcyclelist{mycyclelist}{
% %   basisColor12sw,semithick, every mark/.append style={solid, fill=.},mark=*           \\%
% %   basisColor11sw,semithick, every mark/.append style={solid, fill=.},mark=square*     \\%
% %   basisColor10sw,semithick, every mark/.append style={solid, fill=.},mark=triangle*   \\%
% %   basisColor9sw , semithick,every mark/.append style={solid, fill=.},mark=diamond*    \\%
% %   basisColor8sw , semithick,every mark/.append style={solid, fill=.},mark=otimes    \\%
% % }
% % %% based on "linestyles*", pgfplots documentation S.199
% % % \pgfplotscreateplotcyclelist{mycyclelist}{
% % % semithick,darkgray,solid,        mark=*             \\%
% % % semithick,darkgray,dashed,       mark=square*       \\%
% % % semithick,darkgray,dotted,       mark=triangle*     \\%
% % % semithick,darkgray,dashdotted,   mark=diamond*      \\%
% % % semithick,darkgray,dashdotdotted,mark=otimes        \\%
% % % }
% % % %% copy of "black white", pgfplots documentation S.198 
% % % \pgfplotscreateplotcyclelist{mycyclelist}{
% % % every mark/.append style={fill=gray},mark=*\\%
% % % every mark/.append style={fill=gray},mark=square*\\%
% % % % every mark/.append style={fill=gray},mark=otimes*\\%
% % % mark=star\\%
% % % every mark/.append style={fill=gray},mark=diamond*\\%
% % % densely dashed,every mark/.append style={solid,fill=gray},mark=*\\%
% % % densely dashed,every mark/.append style={solid,fill=gray},mark=square*\\%
% % % % densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
% % % densely dashed,every mark/.append style={solid},mark=star\\%
% % % densely dashed,every mark/.append style={solid,fill=gray},mark=diamond*\\%
% % % }
% % % %% end copy
% % }{

%% red styles
% \pgfplotscreateplotcyclelist{mycyclelist}{
%   basisColor12,semithick,   every mark/.append style={solid, fill=.},mark=*           \\%
%   basisColor11,semithick,   every mark/.append style={solid, fill=.},mark=square*     \\%
%   basisColor10,semithick,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
%   basisColor9, semithick,   every mark/.append style={solid, fill=.},mark=+    \\%
%   basisColor8, semithick,   every mark/.append style={solid, fill=.},mark=otimes    \\%
% }
% % %
% % }

% % %%% Cyclelist 5 comparison for trimmed cube example
% \pgfplotscreateplotcyclelist{mycyclelist}{
% thick,blue,every mark/.append style={fill=blue!80!black},mark=*\\%
% thick,red,dashed,every mark/.append style={fill=red!80!black},mark=square*\\%
% thick,brown!60!black,dashdotted,every mark/.append style={fill=brown!80!black},mark=otimes*\\%
% black,dashed,mark=star\\%
% }


% \definecolor{cyclelistRed}{RGB}{228,26,28}
% \definecolor{cyclelistBlue}{RGB}{55,126,184}
% \definecolor{cyclelistGreen}{RGB}{77,175,74}
% \definecolor{cyclelistViolette}{RGB}{152,78,163}
% \pgfplotscreateplotcyclelist{mycyclelistcompare}{
%   cyclelistRed,     semithick, solid               	\\%
%   cyclelistBlue,    semithick, loosely dashdotted        \\%
%   cyclelistGreen,   semithick, dashed      		\\%
%   cyclelistViolette,semithick, loosely dashdotdotted     \\%
%   cyclelistRed,     only marks,   every mark/.append style={solid, fill=.},mark=*          \\%
%   cyclelistBlue,    only marks,   every mark/.append style={solid, fill=.},mark=square*     \\%
%   cyclelistGreen,   only marks,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
%   cyclelistViolette,only marks,   every mark/.append style={solid, fill=.},mark=diamond*    \\%
% }

%% red and blue styles
% \pgfplotscreateplotcyclelist{mycyclelistcompare}{
%   basisColor1,     semithick, solid               	\\%
%   basisColor10,    semithick, loosely dashdotted        \\%
%   basisColor3,   semithick, dashed      		\\%
%   basisColor12,semithick, loosely dashdotdotted     \\%
%   basisColor1,     only marks,   every mark/.append style={solid, fill=.},mark=*          \\%
%   basisColor10,    only marks,   every mark/.append style={solid, fill=.},mark=square*     \\%
%   basisColor3,   only marks,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
%   basisColor12,only marks,   every mark/.append style={solid, fill=.},mark=diamond*    \\%
% }

% % \ifthenelse{\boolean{isbook}}{ 
% % %% gray styles
% % \pgfplotscreateplotcyclelist{mycyclelistcompare}{
% %   basisColor12sw, semithick, loosely dashdotdotted     \\%
% %   basisColor11sw, semithick, loosely dashed      		\\%
% %   basisColor10sw, semithick, dashed \\%loosely dashdotted        \\%
% %   basisColor9sw,  semithick, solid               	\\%
% %   basisColor12sw, only marks,   every mark/.append style={solid, fill=.},mark=otimes    \\%
% %   basisColor11sw, only marks,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
% %   basisColor10sw, only marks,   every mark/.append style={solid, fill=.},mark=square*     \\%
% %   basisColor9sw,  only marks,   every mark/.append style={solid, fill=.},mark=*          \\%
% % }
% % %
% % 
% % }{
%% red styles
\pgfplotscreateplotcyclelist{mycyclelistcompare}{
  basisColor12, semithick, loosely dashdotdotted     \\%
  basisColor11, semithick, loosely dashed      		\\%
  basisColor10, semithick, dashed \\%loosely dashdotted        \\%
  basisColor9,  semithick, solid               	\\%
  basisColor12, only marks,   every mark/.append style={solid, fill=.},mark=otimes    \\%
  basisColor11, only marks,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
  basisColor10, only marks,   every mark/.append style={solid, fill=.},mark=square*     \\%
  basisColor9,  only marks,   every mark/.append style={solid, fill=.},mark=*          \\%
}
% % %
% % }
%%% Cyclelist 3 (TikZ standard)
\pgfplotscreateplotcyclelist{mycyclelistFastAssL2}{
%     \pgfplotscreateplotcyclelist{color}{%
blue,every mark/.append style={fill=white,scale=1.2},mark=*\\%
red,every mark/.append style={fill=white,scale=1.1},mark=square*\\%
brown!60!black,every mark/.append style={fill=white,scale=1.5},mark=triangle*\\%
black,every mark/.append style={fill=white,scale=1.3},mark=pentagon*\\%
blue,every mark/.append style={fill=white,scale=1.4},mark=diamond*\\%
red,densely dashed,every mark/.append style={solid,fill=white,scale=1.2},mark=*\\%
blue,only marks,every mark/.append style={scale=0.6},mark=*\\%
red,only marks,every mark/.append style={scale=0.55},mark=square*\\%
brown!60!black,only marks,every mark/.append style={scale=0.6},mark=triangle*\\%
black,only marks,every mark/.append style={scale=0.65},mark=pentagon*\\%
blue,only marks,every mark/.append style={scale=0.7},mark=diamond*\\%
red,only marks,every mark/.append style={solid,scale=1.0},mark=star\\%
}

\pgfplotscreateplotcyclelist{mycyclelistFastAssL2Short}{
%     \pgfplotscreateplotcyclelist{color}{%
blue,every mark/.append style={fill=white,scale=1.2},mark=*\\%
red,every mark/.append style={fill=white,scale=1.1},mark=square*\\%
brown!60!black,every mark/.append style={fill=white,scale=1.5},mark=triangle*\\%
black,every mark/.append style={fill=white,scale=1.3},mark=pentagon*\\%
blue,every mark/.append style={fill=white,scale=1.4},mark=diamond*\\%
% red,densely dashed,every mark/.append style={solid,fill=white,scale=1.2},mark=*\\%
blue,only marks,every mark/.append style={scale=0.6},mark=*\\%
red,only marks,every mark/.append style={scale=0.55},mark=square*\\%
brown!60!black,only marks,every mark/.append style={scale=0.6},mark=triangle*\\%
black,only marks,every mark/.append style={scale=0.65},mark=pentagon*\\%
blue,only marks,every mark/.append style={scale=0.7},mark=diamond*\\%
% red,only marks,every mark/.append style={solid,scale=1.0},mark=star\\%
}

\pgfplotscreateplotcyclelist{mycyclelistFastAssEl}{
%     \pgfplotscreateplotcyclelist{color}{%
blue,every mark/.append style={fill=white,scale=1.2},mark=*\\%
red,every mark/.append style={fill=white,scale=1.1},mark=square*\\%
brown!60!black,every mark/.append style={fill=white,scale=1.5},mark=triangle*\\%
% black,every mark/.append style={fill=white,scale=1.3},mark=pentagon*\\%
% blue,every mark/.append style={fill=white,scale=1.4},mark=diamond*\\%
% red,densely dashed,every mark/.append style={solid,fill=white,scale=1.2},mark=*\\%
blue,only marks,every mark/.append style={scale=0.6},mark=*\\%
red,only marks,every mark/.append style={scale=0.55},mark=square*\\%
brown!60!black,only marks,every mark/.append style={scale=0.6},mark=triangle*\\%
black,only marks,every mark/.append style={scale=0.65},mark=pentagon*\\%
blue,only marks,every mark/.append style={scale=0.7},mark=diamond*\\%
% red,only marks,every mark/.append style={solid,scale=1.0},mark=star\\%
}

%%% Cyclelist 3 (TikZ standard)
\pgfplotscreateplotcyclelist{mycyclelist}{
%     \pgfplotscreateplotcyclelist{color}{%
blue,every mark/.append style={fill=blue!80!black},mark=*\\%
red,every mark/.append style={fill=red!80!black},mark=square*\\%
brown!60!black,every mark/.append style={fill=brown!80!black},mark=otimes*\\%
black,mark=star\\%
blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
brown!60!black,densely dashed,every mark/.append style={
solid,fill=brown!80!black},mark=square*\\%
black,densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
blue,densely dashed,mark=star,every mark/.append style=solid\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*\\%
}

% % \ifthenelse{\boolean{isbook}}{ 
% % %% gray styles
% % \tikzset{mycyclelistcompareReferenceA/.style={basisColor12sw,solid}}
% % \tikzset{mycyclelistcompareTestA/.style={basisColor12sw,only marks,mark=otimes}}
% % }{
%% red styles
\tikzset{mycyclelistcompareReferenceA/.style={basisColor12,solid}}
\tikzset{mycyclelistcompareTestA/.style={basisColor12,only marks,mark=otimes}}
% % }
% \pgfplotscreateplotcyclelist{mycyclelistcompareToReference}{
%   basisColor9, very thick, loosely dashed    \\%
%   basisColor12, solid\\%
% %   basisColor11, semithick, loosely dashed      		\\%
% %   basisColor10, semithick, dashed \\%loosely dashdotted        \\%
% %   basisColor9,  semithick, solid               	\\%
% %   basisColor12, only marks,mark=otimes    \\%
% %   basisColor11, only marks,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
% %   basisColor10, only marks,   every mark/.append style={solid, fill=.},mark=square*     \\%
% %   basisColor9,  only marks,   every mark/.append style={solid, fill=.},mark=*          \\%
% }



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Additional styles

%% line styles
\tikzset{helpline/.style={thin,dashed}}
\tikzset{labelline/.style={thin}}
\tikzset{referencePath/.style={dotted,very thick}}
\tikzset{helparrow/.style={thin,arrows={-latex}}}
% \tikzset{pointer/.style={arrows={latex-latex}}}
\tikzset{pointer/.style={arrows={-latex}}}
\tikzset{axis/.style={thin,arrows={->}}}
\tikzset{force/.style={thick,arrows={->}}}
\tikzset{forceInverse/.style={thick,arrows={<-}}}
\tikzset{Gamma/.style={ultra thick}}
\tikzset{controlPoly/.style={draw=black}}
% \tikzset{GammaFill/.style={fill=lightgray,fill opacity=0.3}}
\tikzset{GammaFill/.style={fill=gray,fill opacity=0.3}}
\tikzset{colorDiri/.style={drawgreen}}
\tikzset{GammaFillDiri/.style={fill=drawgreen,fill opacity=0.5}}
% \tikzset{initialgrid/.style={thin,gray}}
\tikzset{initialgrid/.style={thin},darkgray}
\tikzset{intersectioncurve/.style={dashed,thick}}
\tikzset{trimmingcurve/.style={thick}}
\tikzset{boundingbox/.style={dashed,}}
\tikzset{approx/.style={thick,line join=round,dashed}}
\tikzset{integrationRegionEdge/.style={dashed}}

%% point styles
\tikzstyle{anode}= [circle, inner sep=1.3pt, draw, fill=black]
\tikzstyle{gausspoint}=[shape=circle,draw=black,fill=black,inner sep=0.8pt]
\tikzstyle{controlPoint}=[shape=circle,draw=black,fill=white,thin,inner sep=0pt,minimum size=1.5mm]
\tikzstyle{abscissaPoint}=[shape=circle,draw=black,fill=white,thin,inner sep=0pt,minimum size=1.5mm]
\tikzstyle{anchorPoint}=[shape=circle,draw=black,fill=black,thin,inner sep=0pt,minimum size=1.5mm]
% \tikzstyle{anchorPointDeg}=[shape=circle,draw=black,fill=white,thin,inner sep=0pt,minimum size=1.5mm]
\tikzstyle{anchorPointDeg}=[shape=cross out,thick,draw=IFBblue,inner sep=0pt,minimum size=1.5mm]
\tikzstyle{trimmingIntersectionPoint}=[shape=cross out,thick,draw=black,inner sep=0pt,minimum size=1.5mm]
\tikzstyle{approxnode}= [circle, inner sep=1.0pt, draw, fill=black]
% \tikzstyle{characterNode}= [rectangle, inner sep=1.8pt, draw,thick,fill=white]
\tikzstyle{characterNode}= [shape=cross out,rotate=45, inner sep=1.8pt, draw,very thick,fill=white]

\tikzstyle{aPointPatchA}= [circle, inner sep=1.3pt, draw, fill=black]
\tikzstyle{aPointPatchB}= [circle, inner sep=1.3pt, draw, fill=white]
\tikzstyle{aPointModelSpace}=[shape=cross out,thick,draw=black,inner sep=0pt,minimum size=1.5mm]


% \tikzstyle{anchorPoint}=[shape=circle,draw=black,fill=black,inner sep=0pt,minimum size=1.5mm]%, maximum size=1.5mm]
% \tikzstyle{anchorPointDisp}=[shape=circle,draw=black,fill=drawgreen,inner sep=0pt,minimum size=1.5mm]%, maximum size=1.5mm]
% \tikzstyle{collocPoint}=[shape=rectangle,draw=black,fill=black,thick,inner sep=0pt,minimum size=1.2mm] %, maximum size=1.2mm] 
% \tikzset{Diri/.style={drawgreen}}
% \tikzset{Neum/.style={drawpurple}}
% \tikzset{collocNeum/.style={collocPoint, fill=drawgreen}}
% \tikzset{collocDiri/.style={collocPoint, fill=drawpurple}}
% 
% \tikzset{GammaDiri/.style={Gamma, Diri}}
% \tikzset{GammaNeum/.style={Gamma, Neum}}
% 
% \tikzset{anchorNeum/.style={anchorPoint, fill=drawpurple}}
% \tikzset{anchorDiri/.style={anchorPoint, fill=drawgreen}}
% 
% \tikzset{helpline/.style={thin,dashed}}
% \tikzset{helpline/.style={thin}}

%% rotation for 3D plots
\newcommand{\rotateRPY}[3]% roll, pitch, yaw
{   \pgfmathsetmacro{\rollangle}{#1}
    \pgfmathsetmacro{\pitchangle}{#2}
    \pgfmathsetmacro{\yawangle}{#3}

    % to what vector is the x unit vector transformed, and which 2D vector is this?
    \pgfmathsetmacro{\newxx}{cos(\yawangle)*cos(\pitchangle)}
    \pgfmathsetmacro{\newxy}{sin(\yawangle)*cos(\pitchangle)}
    \pgfmathsetmacro{\newxz}{-sin(\pitchangle)}
    \path (\newxx,\newxy,\newxz);
    \pgfgetlastxy{\nxx}{\nxy};

    % to what vector is the y unit vector transformed, and which 2D vector is this?
    \pgfmathsetmacro{\newyx}{cos(\yawangle)*sin(\pitchangle)*sin(\rollangle)-sin(\yawangle)*cos(\rollangle)}
    \pgfmathsetmacro{\newyy}{sin(\yawangle)*sin(\pitchangle)*sin(\rollangle)+ cos(\yawangle)*cos(\rollangle)}
    \pgfmathsetmacro{\newyz}{cos(\pitchangle)*sin(\rollangle)}
    \path (\newyx,\newyy,\newyz);
    \pgfgetlastxy{\nyx}{\nyy};

    % to what vector is the z unit vector transformed, and which 2D vector is this?
    \pgfmathsetmacro{\newzx}{cos(\yawangle)*sin(\pitchangle)*cos(\rollangle)+ sin(\yawangle)*sin(\rollangle)}
    \pgfmathsetmacro{\newzy}{sin(\yawangle)*sin(\pitchangle)*cos(\rollangle)-cos(\yawangle)*sin(\rollangle)}
    \pgfmathsetmacro{\newzz}{cos(\pitchangle)*cos(\rollangle)}
    \path (\newzx,\newzy,\newzz);
    \pgfgetlastxy{\nzx}{\nzy};
}

\tikzset{RPY/.style={x={(\nxx,\nxy)},y={(\nyx,\nyy)},z={(\nzx,\nzy)}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% help macro for convergence plots

\def\trianglecolor{black}
\newcommand{\upperSlopeTriangle}[4] 	% input: #1 slope #2 vertical shift  #3 min x-value #4 max x-value
								% example call: \upperSlopeTriangle{2}{100}{1000}{5000}
{
	\addplot[forget plot, domain=#3:#4,color=\trianglecolor,samples=2]{  #2 / (x^#1) } node (A1) [pos=1] {}; 
	\addplot[forget plot, domain=#3:#4,color=\trianglecolor,samples=2]{   #2  / (#3^#1)} node (A2) [pos=1] {} node [anchor=south,pos=0.5,black] {\tikzfontsizetiny $1$};
	\draw[color=\trianglecolor] (A1.center) -- (A2.center) node [anchor=west,pos=0.5,black] {\tikzfontsizetiny #1};
}

\newcommand{\upperSlopeTriangleFlip}[4] 	% input: #1 slope #2 vertical shift  #3 min x-value #4 max x-value
								% example call: \upperSlopeTriangle{2}{100}{1000}{5000}
{
	\addplot[forget plot, domain=#3:#4,color=\trianglecolor,samples=2]{  #2 / (x^-#1) } node (A1) [pos=1] {}; 
	\addplot[forget plot, domain=#3:#4,color=\trianglecolor,samples=2]{  #2 / (#3^-#1)} node (A2) [pos=1] {} node [anchor=north,pos=0.5,black] {\tikzfontsizetiny $1$};
	\draw[color=\trianglecolor] (A1.center) -- (A2.center) node [anchor=west,pos=0.5,black] {\tikzfontsizetiny #1};
}

\newcommand{\lowerSlopeTriangle}[4] 	% input: #1 slope #2 vertical shift  #3 min x-value #4 max x-value
								% example call: \lowerSlopeTriangle{2}{100}{1000}{5000}
{
% 	\def\trianglecolor{black}
	\addplot[forget plot, domain=#3:#4,color=\trianglecolor,samples=2]{  #2 / (x^#1) } node (A1) [pos=0] {}; 
	\addplot[forget plot, domain=#3:#4,color=\trianglecolor,samples=2]{   #2  / (#4^#1)} node (A2) [pos=0] {} node [anchor=north,pos=0.5,black] {\tikzfontsizetiny $1$};
	\draw[color=\trianglecolor] (A1.center) -- (A2.center) node [anchor=east,pos=0.5,black] {\tikzfontsizetiny #1};
}
\newcommand{\lowerSlopeTriangleFlip}[4] 	% input: #1 slope #2 vertical shift  #3 min x-value #4 max x-value
								% example call: \lowerSlopeTriangle{2}{100}{1000}{5000}
{
% 	\def\trianglecolor{black}
	\addplot[forget plot, domain=#3:#4,color=\trianglecolor,samples=2]{  #2 / (x^-#1) } node (A1) [pos=0] {}; 
	\addplot[forget plot, domain=#3:#4,color=\trianglecolor,samples=2]{   #2  / (#4^-#1)} node (A2) [pos=0] {} node [anchor=south,pos=0.5,black] {\tikzfontsizetiny $1$};
	\draw[color=\trianglecolor] (A1.center) -- (A2.center) node [anchor=east,pos=0.5,black] {\tikzfontsizetiny #1};
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% tikz helper functions

%% add a picture to a tikz figure
% #1... picture name
% #2... figure options (e.g., "scale=\tkzscale,angle=0")
% #3... grid on if value is 1
% #4... extra tikz elements
% #5... clipping commands
%
%% Example call
%   \myaddgraphic{trimmedPatch}{scale=\tkzscale}{0} % set to 1 to turn help grid on
%   { % add nodes
%       \draw (0.11,0.21) rectangle (0.93,0.86);  
%   }{% add clipping 
%       \clip (0.11,0.21) rectangle (0.93,0.86);  
%   }
\newcommand{\myaddgraphic}[5]
{
 \node[anchor=south west,inner sep=0] (image) {\phantom{\includegraphics[#2]{#1}}};
  \begin{scope}[x={(image.south east)},y={(image.north west)}]
      
      \begin{scope}
          
          #5
          
          \node[anchor=south west,inner sep=0] {\includegraphics[#2]{#1}};
      \end{scope} 
      
      #4
      
      \pgfmathparse{int(#3)} \let\gridIndicator\pgfmathresult
      \ifthenelse{ \gridIndicator = 1 }
      {
          %% help lines
          \draw[help lines,xstep=.1,ystep=.1] (0,0) grid (1.001,1.001);
          \foreach \x in {1,...,9} { \node [anchor=north] at (\x/10,0) {\x};}
          \foreach \y in {1,...,9} { \node [anchor=east] at (0,\y/10) {\y};}
      }{}
      
  \end{scope}    
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Bezier curven -- control points
\usetikzlibrary{decorations.pathreplacing,backgrounds}
% example call: \draw[show curve controls={blue}{red}] (A) .. controls (B) and (C) .. (D);
\tikzset{
  show curve controls/.style n args={2}{
    decoration={
      show path construction,
      curveto code={
        \draw[#1]
        (\tikzinputsegmentfirst)
        -- (\tikzinputsegmentsupporta)
        -- (\tikzinputsegmentsupportb)
        -- (\tikzinputsegmentlast)
        ;
        \fill[#1] (\tikzinputsegmentsupporta) circle(1pt);
        \fill[#1] (\tikzinputsegmentsupportb) circle(1pt);
        \draw[#2]
        (\tikzinputsegmentfirst)
        .. controls (\tikzinputsegmentsupporta)
                and (\tikzinputsegmentsupportb) ..
        (\tikzinputsegmentlast);
      }
    },decorate
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% B-spline functions



\newcounter{itR}
\newcommand{\bsplinevalue}[5] % input: #1 knot vector #2 order,  #3 intrinsic coordinate #4 span index #5 output name
						% remark: #1 has to be parsed explicitly ( \def\vKnots{...} \bsplinevalue{\vKnots}{×}{×}{×}{×} fails!  )
{                    				
	\newarray\vKnots
	\newarray\vN
	\newarray\vNumeratorL
	\newarray\vNumeratorR
	\newarray\vSave

	\readarray{vKnots}{#1}
	\readarray{vN}{1}
	\readarray{vSave}{0}
	\readarray{vNumeratorL}{0}
	\readarray{vNumeratorR}{0}

	\foreach \j in {1,...,#2}
	{        
		\pgfmathparse{ int(#4+\j+1) } \checkvKnots(\pgfmathresult)
		\pgfmathsetmacro{\numR}{\cachedata-#3}
		
		\pgfmathparse{ int(#4-\j+2) } \checkvKnots(\pgfmathresult)
		\pgfmathsetmacro{\numL}{#3-\cachedata} 					

		\expandarrayelementtrue
		\pgfmathparse{ int(\j+1) }
		\vNumeratorL(\pgfmathresult)={\numL}
		\vNumeratorR(\pgfmathresult)={\numR}
		
		\forloop[1]{itR}{0}{\value{itR} < \j }
		{
			\pgfmathparse{ int(\theitR+1) } \let\tS\pgfmathresult  	
			\checkvSave(\tS)							
			\pgfmathsetmacro{\save}{\cachedata}  
		
			\pgfmathparse{int(\j-\theitR+1)} \checkvNumeratorL(\pgfmathresult)
			\pgfmathsetmacro{\tmpL}{\cachedata} 	
		    
			\pgfmathparse{ int(\theitR+2) } \checkvNumeratorR(\pgfmathresult)
			\pgfmathsetmacro{\tmpR}{\cachedata} 	       
	
			\pgfmathparse{ int(\theitR+1) } \checkvN(\pgfmathresult)
			\pgfmathparse{ \cachedata / (\tmpL+\tmpR) } \let\tmp\pgfmathresult
			
			\pgfmathparse{ \save + \tmpR * \tmp } 
			\vN(\tS)={\pgfmathresult}

			\pgfmathparse{ \tmpL * \tmp } \let\tmpsave\pgfmathresult
			\pgfmathparse{ int(\theitR+2) } \let\tS\pgfmathresult      
			\vSave(\tS)={\tmpsave}
		}
		
		\pgfmathparse{ int(\j+1) } \checkvSave(\pgfmathresult )
		\vN(\tS)={\cachedata}
	}

	% write to return argument #5
	\pgfmathparse{int( #2+1) } \let\lastIndex\pgfmathresult
	\checkvN(1) \pgfmathsetmacro{\first}{\cachedata}  
	\foreach \i [remember=\a as \lasta (initially \first)] in {2,...,\lastIndex}
	{
		\checkvN(\i) \def\a{\lasta,\cachedata} 
		% store \a of last loop
		\ifthenelse{\i=\lastIndex}{ \xdef#5{\a} }{}
	}
    
	% clean up
	\foreach \i in {1,...,\lastIndex}
	{
	    \clrarray{vNumeratorR}(\i)
	    \clrarray{vNumeratorL}(\i)
	    \clrarray{vN}(\i)
	    \clrarray{vSave}(\i)
	}
	\delarray\vN
	\delarray\vNumeratorL
	\delarray\vNumeratorR
	\delarray\vSave
}

\newcounter{countvalues}
\newcounter{getBasis}
\newcommand{\bsplinebasis}[4] % input: #1 knot vector, #2 order,  #3 id of basis function, #4 output
{						% example: \bsplinebasis{0&0&0&1&2&2&2}{2}{0}{\output}
						% remark: #1 has to be parsed explicitly ( \def\vKnots{...} \bsplinebasis{\vKnots}{×}{×}{×} fails!  )
						%		countvalues returns the number of non-zero basis functions
						%		\output ''intrinsic Coord, basis function value'': ''u0,N_#3(u0)'',''u1,N_#3(u1)'',...,''un,N_#3(un)''
    \newarray\vKnots 	% remark index start from 1
    \readarray{vKnots}{#1}

    \pgfmathparse{#3}  \let\i\pgfmathresult
    \pgfmathparse{#2}  \let\p\pgfmathresult

    % loop over support of N_i
    \setcounter{countvalues}{0}
    \setcounter{getBasis}{\p} %\addtocounter{getBasis}{1}
    \pgfmathparse{int(\i+\p)}
    \foreach \knotspan in {\i,...,\pgfmathresult}
    {
        % check span size
	\pgfmathparse{ int(\knotspan+1+1) } \checkvKnots(\pgfmathresult)
	\pgfmathsetmacro{\tmpR}{\cachedata} 						%R: \tmpR
	
	\pgfmathparse{ int(\knotspan+1) } \checkvKnots(\pgfmathresult) 
	\pgfmathsetmacro{\tmpL}{\cachedata} 						%L: \tmpL

	\pgfmathparse{ \tmpR - \tmpL } \let\spansize\pgfmathresult  			%S: \spansize 
   
        \pgfmathparse{ \spansize > 0.0 } \let\bNonZero\pgfmathresult
        \ifthenelse{ \bNonZero = 1 }
        {
            % evaluate points \u with in the span
            \foreach \percentU in {0,10,...,100}
            {
		\pgfmathparse{\tmpL+\spansize*\percentU/100} \let\u\pgfmathresult

		% get all non vanishing basis functions
		\bsplinevalue{#1}{\p}{\u}{\knotspan}{\Basis} 
		\def\basisfuncarray{{\Basis}} 				% remark index start from 0
		
		\pgfmathparse{\basisfuncarray[\thegetBasis]} %\pgfmathresult
		
		\ifthenelse{\thecountvalues=0}
		{ 
			\xdef\nodeB{"\u,\pgfmathresult"}
		}{
			\xdef\nodeB{\nodeB,"\u,\pgfmathresult"}  
		}
		\addtocounter{countvalues}{1}
            }
        }{}
        \addtocounter{getBasis}{-1}
    }
    
	\xdef#4{\nodeB}

	\delarray\vKnots
}


\newcommand{\bsplinebasisspan}[6] % input: 	#1 knot vector, #2 order,  #3 segment id of basis function within (#4), 
{							% 		#4 id of knot span,  #5 id of plotted span, #6 output
							% example: \bsplinebasis{0&0&0&1&2&2&2}{2}{0}{\output}
							% remark: #1 has to be parsed explicitly ( \def\vKnots{...} \bsplinebasis{\vKnots}{×}{×}{×} fails!  )
							%		#3 is not  the basis function id 
							%		   - for each span the numbering start at 0 - index first non-zero basis function of #4
							%		countvaluesspan returns the number of non-zero basis functions
							%		\output ''intrinsic Coord, basis function value'': ''u0,N_#3(u0)'',''u1,N_#3(u1)'',...,''un,N_#3(un)''
    \newarray\vKnots 	% remark index start from 1
    \readarray{vKnots}{#1}

    \pgfmathparse{#5}  \let\plotknotspan\pgfmathresult
    \pgfmathparse{#4}  \let\splineknotspan\pgfmathresult
    \pgfmathparse{#3}  \let\i\pgfmathresult
    \pgfmathparse{#2}  \let\p\pgfmathresult

    % only one iteration over support '\plotknotspan' 
    % evaluation the polynome defined over '\splineknotspan'
    \setcounter{countvalues}{0}
    \setcounter{getBasis}{\i} 
    \foreach \knotspan in {\plotknotspan}
    {
        % check span size
	\pgfmathparse{ int(\knotspan+1+1) } \checkvKnots(\pgfmathresult)
	\pgfmathsetmacro{\tmpR}{\cachedata} 						%R: \tmpR
	
	\pgfmathparse{ int(\knotspan+1) } \checkvKnots(\pgfmathresult) 
	\pgfmathsetmacro{\tmpL}{\cachedata} 						%L: \tmpL

	\pgfmathparse{ \tmpR - \tmpL } \let\spansize\pgfmathresult  			%S: \spansize 
   
        \pgfmathparse{ \spansize > 0.0 } \let\bNonZero\pgfmathresult
        \ifthenelse{ \bNonZero = 1 }
        {
            % evaluate points \u with in the span
            \foreach \percentU in {0,10,...,100}
            {
		\pgfmathparse{\tmpL+\spansize*\percentU/100} \let\u\pgfmathresult

		% get all non vanishing basis functions
		\bsplinevalue{#1}{\p}{\u}{\splineknotspan}{\Basis} 
		\def\basisfuncarray{{\Basis}} 				% remark index start from 0
		
		\pgfmathparse{\basisfuncarray[\thegetBasis]} %\pgfmathresult
		
		\ifthenelse{\thecountvalues=0}
		{ 
			\xdef\nodeB{"\u,\pgfmathresult"}
		}{
			\xdef\nodeB{\nodeB,"\u,\pgfmathresult"}  
		}
		\addtocounter{countvalues}{1}
            }
        }{}
        \addtocounter{getBasis}{-1}
    }
    
	\xdef#6{\nodeB}

	\delarray\vKnots
}





\newcommand{\plotbsplinebasis}[4] 	% input: #1 knot vector, #2 order,  #3 id of basis function, #4 plot settings
{							% example: \plotbsplinebasis{0&0&0&1&2&2&2}{2}{0}{green,smooth}
							% remark: #1 has to be parsed explicitly ( \def\vKnots{...} \plotbsplinebasis{\vKnots}{×}{×}{×} fails!  )
	% calculate B-spline values
	\bsplinebasis{#1}{#2}{#3}{\nodeOut}
	\def\nodearray{{\nodeOut}}

	% store B-spline values into coordinates and save their name
	\xdef\name{ }
	\addtocounter{countvalues}{-1}
	\foreach \i in {0,...,\thecountvalues}
	{
		\pgfmathparse{\nodearray[\i]}
		\coordinate (point\i) at (\pgfmathresult);	  
		\xdef\name{ \name (point\i)  }
	}
	
	% plot basis
	\draw[#4] plot coordinates{ \name };
	
	% reset coordinates
	\xdef\name{ }
}


\newcommand{\plotbsplinesegment}[6] 	% input: 	#1 knot vector, #2 order,  #3 segment id of basis function within (#4),  
{								%		#4 id of knot span, #5 id of plotted span, #6 plot settings
								% example: 
								%	->normal B-spline plot
								% 	\plotbsplinebasis{0&0&0&1&2&3&3&3}{2}{1}{basisColor3,dotted,thick}
								%	\plotbsplinebasis{0&0&0&1&2&3&3&3}{2}{2}{basisColor5,dotted,thick}
								%	\plotbsplinebasis{0&0&0&1&2&3&3&3}{2}{3}{basisColor7,dotted,thick}
								%	
								%	-> plot the B-spline segments 0,1,2 of span 3 in span 2
								%
								%	\plotbsplinesegment{0&0&0&1&2&3&3&3}{2}{0}{3}{2}{red,smooth}
								%	\plotbsplinesegment{0&0&0&1&2&3&3&3}{2}{1}{3}{2}{red,smooth}
								%	\plotbsplinesegment{0&0&0&1&2&3&3&3}{2}{2}{3}{2}{blue,smooth}
								%
								% remark: #1 has to be parsed explicitly ( \def\vKnots{...} \plotbsplinebasis{\vKnots}{×}{×}{×} fails!  
								
	% calculate B-spline values
	\bsplinebasisspan{#1}{#2}{#3}{#4}{#5}{\nodeOut}
	\def\nodearray{{\nodeOut}}

	% store B-spline values into coordinates and save their name
	\xdef\name{ }
	\addtocounter{countvalues}{-1}
	\foreach \i in {0,...,\thecountvalues}
	{
		\pgfmathparse{\nodearray[\i]}
		\coordinate (point\i) at (\pgfmathresult);	  
		\xdef\name{ \name (point\i)  }
	}
	
	% plot basis
	\draw[#6] plot coordinates{ \name };
	
	% reset coordinates
	\xdef\name{ }
}


\newcommand{\plotbsplineaccumulated}[5] 	% input: 	#1 knot vector, #2 order,  #3 subdivision coefficient,  
{						%		#4 id of knot span,  #5 plot settings
						% example: 
                                                %       ->plot non-zero basis function segment within #4
						%	\plotbsplineaccumulated{0&0&0&1&2&3&3&3}{2}{1&0&0}{3}{red,smooth}
						% 	\plotbsplineaccumulated{0&0&0&1&2&3&3&3}{2}{0&1&0}{3}{green,smooth}
						%	\plotbsplineaccumulated{0&0&0&1&2&3&3&3}{2}{0&0&1}{3}{blue,smooth}
                                                %       
                                                %       ->plot weighted combination of basis function segments within #4
						%	\plotbsplineaccumulated{0&0&0&1&2&3&3&3}{2}{0&1&1}{3}{blue,smooth}
						%	
						% remark: #1 has to be parsed explicitly ( \def\vKnots{...} \plotbsplinebasis{\vKnots}{×}{×}{×} fails!  

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%                                                            
    %% calculate B-spline values and compute their weighted sum using vSubCoef
    \newarray\vKnots 	% remark index start from 1
    \readarray{vKnots}{#1}
    \newarray\vSubCoef 	% remark index start from 1
    \readarray{vSubCoef}{#3}
    
    \pgfmathparse{#4}  \let\plotknotspan\pgfmathresult
    \pgfmathparse{#4}  \let\splineknotspan\pgfmathresult
    \pgfmathparse{#2}  \let\p\pgfmathresult
    
    % only one iteration over support '\plotknotspan' 
    % evaluation the polynome defined over '\splineknotspan'
    \setcounter{countvalues}{0}
    \pgfmathparse{int( \p+1) } \let\lastIndex\pgfmathresult
    \foreach \knotspan in {\plotknotspan}
    {
        % check span size
        \pgfmathparse{ int(\knotspan+1+1) } \checkvKnots(\pgfmathresult)
        \pgfmathsetmacro{\tmpR}{\cachedata} 						%R: \tmpR
        
        \pgfmathparse{ int(\knotspan+1) } \checkvKnots(\pgfmathresult) 
        \pgfmathsetmacro{\tmpL}{\cachedata} 						%L: \tmpL
        
        \pgfmathparse{ \tmpR - \tmpL } \let\spansize\pgfmathresult  			%S: \spansize 
        
        \pgfmathparse{ \spansize > 0.0 } \let\bNonZero\pgfmathresult
        \ifthenelse{ \bNonZero = 1 }
        {
            % evaluate points \u with in the span
            \foreach \percentU in {0,10,...,100}
            {
                \pgfmathparse{\tmpL+\spansize*\percentU/100} \let\u\pgfmathresult
                
                % get all non vanishing basis functions
                \bsplinevalue{#1}{\p}{\u}{\splineknotspan}{\Basis} 
                \def\basisfuncarray{{\Basis}} 				% remark index start from 0
                
                \setcounter{getBasis}{0} 
                \pgfmathparse{\basisfuncarray[\thegetBasis]} %\pgfmathresult
                \let\basisValue\pgfmathresult
                
                \checkvSubCoef(1) \pgfmathsetmacro{\coef}{\cachedata}  
                \pgfmathparse{ \basisValue * \coef } \let\first\pgfmathresult
                
                \xdef\lastx{\first}
                \foreach \i in {2,...,\lastIndex}
                { 
                    \addtocounter{getBasis}{1}       
                    \pgfmathparse{\basisfuncarray[\thegetBasis]}
                    \let\basisValue\pgfmathresult
                    
                    \checkvSubCoef(\i) \pgfmathsetmacro{\coef}{\cachedata}  
                    \pgfmathparse{ \lastx + \basisValue * \coef } \let\sum\pgfmathresult
                    
                    \xdef\lastx{\sum}
                    
                    % store \a of last loop
                    \ifthenelse{\i=\lastIndex}
                    {
                        \ifthenelse{\thecountvalues=0}
                        { 
                            \xdef\nodeBB{"\u,\sum"}
                        }{
                            \xdef\nodeBB{\nodeBB,"\u,\sum"}  
                        }
                        \addtocounter{countvalues}{1}
                    }{}
                    
                }
            }
        }{}
    }
    
    \delarray\vKnots
    \delarray\vSubCoef
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%
    %% plot accumulated values
    \def\nodearray{{\nodeBB}}
    
    % store B-spline values into coordinates and save their name
    \xdef\name{ }
    \addtocounter{countvalues}{-1}
    \foreach \i in {0,...,\thecountvalues}
    {
        \pgfmathparse{\nodearray[\i]}
        \coordinate (point\i) at (\pgfmathresult);                
        \xdef\name{ \name (point\i)  }
    }
    
    % plot basis
    \draw[#5] plot coordinates{ \name };
    
    % reset coordinates
    \xdef\name{ }
}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "mainPhD"
%%% End: 

